Field-Based Toolpath Generation for 3D Printing Continuous Fibre Reinforced Thermoplastic Composites

We present a field-based method of toolpath generation for 3D printing continuous fibre reinforced thermoplastic composites. Our method employs the strong anisotropic material property of continuous fibres by generating toolpaths along the directions of tensile stresses in the critical regions. Moreover, the density of toolpath distribution is controlled in an adaptive way proportionally to the values of stresses. Specifically, a vector field is generated from the stress tensors under given loads and processed to have better compatibility between neighboring vectors. An optimal scalar field is computed later by making its gradients approximate the vector field. After that, isocurves of the scalar field are extracted to generate the toolpaths for continuous fibre reinforcement, which are also integrated with the boundary conformal toolpaths in user selected regions. The performance of our method has been verified on a variety of models in different loading conditions. Experimental tests are conducted on specimens by 3D printing continuous carbon fibres (CCF) in a polylactic acid (PLA) matrix. Compared to reinforcement by load-independent toolpaths, the specimens fabricated by our method show up to 71.4% improvement on the mechanical strength in physical tests when using the same (or even slightly smaller) amount of continuous fibres.

==> Text/Sec3MaterialTest.tex <==






\section{Criterion of CCF Placement: An Experiment Exploration}
\label{sec:experimentalVerification}

\begin{table*}[t]
\centering \footnotesize 
\begin{tabular}{c||cc|cccc|cccc}
\hline \hline
\specialrule{0em}{2pt}{1pt}
\multirow{2}{*}{Specimen} & \multicolumn{2}{c|}{PLA} & \multicolumn{4}{c|}{ PLA (Zig-Zag) + CCF} & \multicolumn{4}{c}{ PLA (Stress-oriented) + CCF} \\ \specialrule{0em}{1pt}{1pt}  \cline{2-11} \specialrule{0em}{1pt}{1pt} 
                          & A           & B          & C       & D       & E       & F       & G         & H         & I          & J         \\ \specialrule{0em}{1pt}{1pt} \hline \specialrule{0em}{1pt}{1pt}
CCF Length (mm)         & N/A         & N/A        & 835.2        & 815.4        & 789.3        & 764.1         & 835.2        & 815.4        & 789.3        & 764.1           \\
Breaking Force (kN)       & 1.36        & 1.57       & 1.49    & 2.11    & 2.90    & 3.98    & 1.52      & 2.25      & 3.58       & 4.62    \\
Young's Modulus (MPa)     & 3,282       & 3,754      & 4,142   & 5,917   & 8,558   & 12,447  & 4,317     & 6,284     & 10,110     & 13,673  \\
\specialrule{0em}{1pt}{1pt} \hline \hline
\end{tabular}
\end{table*}

\begin{figure*}[t]
\includegraphics[width=\linewidth]{images/materialSampleTest.jpg}
\caption{Material samples with different toolpath design. Specimen A, B are use PLA material only, and C - J are printed with composite material. The corresponding breaking force and Young's Modulus under tensile test are present in Table. Notice that all the data are take the average from 3 tests.}
\label{fig:tensileBar}
\end{figure*}

In this section, the reinforcement behavior of CCF is studied. Experiment data is used to quantitative analysis the effectiveness of CCF-reinforcement affected by toolpath design. A series material test is conducted on samples fabricated with various CCF placement strategy. As a brief summary, CCF have higher ability in strengthening model under tensile stress than compression, meanwhile shows a $3 \times$ difference in the breaking force and Young's Modulus (tensile case), with same amount of CCF is used. The criterion of CCF placement is then summarized and used to guide our computation process in design the toolpath. Here we first the experiment below. \charlie{need to rephrase by using the description in \cite{Li2020_CompositeB} as a reference} \singa{This section would be rewrite after discussion with Guoxin}

As is known to all, continuous carbon fibres have several advantages including high stiffness and high tensile strength. Previous work~\cite{Tian16_composite,heidari2019mechanical,TIAN17_JCP,Omuro17_Composite} demonstrates these advantages by conducting tensile test where the specimens with continuous carbon fibres printed along the stress direction are much more stiff and stronger than the neat specimens. However, only a few work has done the compression tests to see if the added continuous carbon fibres can change the behavior of compressive strength. In this work, we aim to reinforce the printed models by taking advantage of the high tensile strength of continuous carbon fibre, therefore we assume that the added continuous carbon fibres have little effect on the compressive strength of the models.
To verify this hypothesis, a cuboid model is selected for compression test since the buckling could be avoided to a certain extent due to the square section.
On the other hand, a series tensile tests would be conducted on a specimen with standard cross-section to detect the influence of different toolpath design for both CCF and PLA. We divide the printed specimens in to three experimental group to explore the influence of each individual variable.

%\guoxin{We first present the preparation of material samples used for material test.} 
As a material have high anisotropic behavior under tensile loading, we first test the behavior on CCF in tensile bar samples. As shows in Fig.~\ref{fig:tensileBar}, 10 material bar were prepared and fabricated by FDM printing. Here sample A and B were fabricated with basement material only (PLA in this test), and sample C - J were fabricate with composite material. Four different CCF toolpath is designed, which includes widely used zig-zag (sample C and G), boundary-contour toolpath (sample D and H), stress-direction toolpath (sample E and I), and stress-oriented toolpath with density control (sample F and J). On the other hand, sample C-F and G-J share different toolpath for base material, where the former one is cross-direction zig-zag and stress oriented for the later one. Note that the length of the CCF consumed in each specimens is controled in a similar leverl as presented in Table 1. 
\guoxin{also add the material model of compression test.}\charlie{why not adding the results of compression?}\singa{shown in Fig.~\ref{fig:Result_Compress&Tensile}}

\begin{figure}[t]
\label{fig:Result_Compress&Tensile}
\includegraphics[width=\linewidth]{images/tensileCompressCompare.png}
\caption{Comparison of CCF-reinforcement effectiveness on tensile and compression. We can observe the enhancement of the breaking force with 329.9\%(in tensile tests) and 114.8\%(in compression tests) when aligning filaments along the direction of loading and considering the distribution of stress.\charlie{It is unclear to me which is which? also for the red curve, why it is a range instead of a curve?}\singa{Changes have been made in PPT, both of them are range, the blue is stable that the curves are almost similar.}\singa{separate version is uploaded}}
\end{figure}

%\guoxin{Material test Result}
We conduct the tensile test on the Landmark® Servohydraulic Test System as illustrated on the right side of Figure.~\ref{figMaterialSampleTest}(a) and list the experiment result on the Table in Fig.~\ref{fig:tensileBar}. We present the result of group G-J in Fig.3. By compare the data from all physical experiment, we got several conclusion to guide the toolpath design for CCF composite printing.

\begin{itemize}
    \item The CCF-reinforcement shows significantly better performance in enhance the stiffness of model under tensile loading than compression. Comparing specimen A and specimen J, it shows a $194 \%$ and $210 \%$ enhancement in breaking force and Young's Modulus, respectively. However, only $10 \%$ increase is detected in compression case (specimen K v.s. specimen L).
   
   \item \charlie{any point missing here?}
   
\end{itemize}

\charlie{I would expect some conclusion about the rules / heuristics of toolpath generation can be made here.}
